In-context Example Selection with Influences

In-context learning (ICL) is a powerful paradigm emerged from large language models (LLMs). Despite its promises, ICL performance is known to be highly sensitive to input examples. In this work, we use $\textit{in-context influences}$ to analyze few-shot ICL performance directly from the in-context examples. Our proposed influence-based example selection method can identify both positive and negative examples, outperforming several baselines when evaluated on 9 SuperGLUE tasks. Our analysis uncovers up to a $16.3\%$ performance gap between using the most negative in-context examples compared to the most positive. In a case study, we apply our influence-based framework to quantify the phenomena of recency bias in example ordering for few-shot ICL.

==> fables/fig_datamodels.tex <==
\begin{figure*}[t]
% \caption{A simple linear in-context datamodel \textit{can} map an arbitrary subset $S'$ to ICL performance.\footnote{See \cref{fig_datamodels-full} in Appendix \cref{appendix:datamodels} for all visualizations}}
\centering
\centerline{\includegraphics[width=1.0\textwidth]{figures/datamodels.png}}
\caption{A simple linear in-context datamodel \textit{can} map an arbitrary subset $S'$ to ICL performance.}
\label{fig_datamodels}
\end{figure*}

==> fables/tab_datamodel-pearson.tex <==

\begin{table*}[htb]
\caption{Pearson correlations (p-value) between actual outputs and linear models' predicted outputs. Bold values are statistically significant up to 0.05.}
\label{tab_datamodel-pearson}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llllllr}
\toprule
{} &               GPT2-XL &                 GPT-J &              OPT-6.7B &               OPT-13B &              GPT-NeoX &               OPT-30B \\
\midrule
piqa              &  \textbf{0.27} (0.00) &  \textbf{0.24} (0.00) &          -0.02 (0.89) &  \textbf{0.24} (0.00) &  \textbf{0.17} (0.03) &  \textbf{0.18} (0.03) \\
boolq   &  \textbf{0.55} (0.00) &  \textbf{0.44} (0.00) &          -0.02 (0.81) &           0.11 (0.12) &  \textbf{0.26} (0.00) &  \textbf{0.37} (0.00) \\
rte     &  \textbf{0.12} (0.01) &  \textbf{0.31} (0.00) &           0.05 (0.64) &  \textbf{0.22} (0.00) &  \textbf{0.19} (0.00) &          -0.01 (0.85) \\
wic     &  \textbf{0.17} (0.00) &           0.05 (0.55) &  \textbf{0.27} (0.04) &           0.14 (0.09) &          0.00 (0.97) &           0.18 (0.06) \\
wsc     &  \textbf{0.16} (0.00) &           0.09 (0.20) &           0.19 (0.14) &           0.04 (0.59) &           0.05 (0.50) &           0.14 (0.08) \\
\midrule
cb      &  \textbf{0.17} (0.00) &  \textbf{0.29} (0.00) &  \textbf{0.36} (0.00) &  \textbf{0.15} (0.00) &           0.02 (0.68) &  \textbf{0.21} (0.00) \\
arc (challenge) &  \textbf{0.29} (0.00) &  \textbf{0.30} (0.00) &           0.15 (0.08) &           0.05 (0.53) &  \textbf{0.29} (0.00) &  \textbf{0.22} (0.01) \\
arc (easy)      &  \textbf{0.31} (0.00) &  \textbf{0.22} (0.01) &  \textbf{0.21} (0.02) &  \textbf{0.30} (0.00) &           0.14 (0.07) &           0.02 (0.81) \\
hellaswag         &  \textbf{0.58} (0.00) &  \textbf{0.55} (0.00) &  \textbf{0.50} (0.00) &  \textbf{0.49} (0.00) &  \textbf{0.62} (0.00) &  \textbf{0.57} (0.00) \\
openbookqa        &  \textbf{0.38} (0.00) &  \textbf{0.23} (0.01) &  \textbf{0.23} (0.01) &  \textbf{0.28} (0.00) &  \textbf{0.32} (0.00) &  \textbf{0.22} (0.01) \\
\midrule
Overall  &  \textbf{0.94} (0.00) &  \textbf{0.94} (0.00)  &  \textbf{0.68} (0.00)  &  \textbf{0.94} (0.00)  &  \textbf{0.95} (0.00)  &  \textbf{0.95} (0.00) \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


==> fables/tab_datamodel-spearman.tex <==
\begin{table*}[ht]
\caption{Spearman correlations (p-value) between actual outputs and linear models' predicted outputs. Bold values are statistically significant up to 0.05.}
\label{tab_datamodel-spearman}
\vskip 0.1in
\begin{center}
% \begin{small}
\begin{sc}
\begin{tabular}{llllllr}
\toprule
{} &               GPT2-XL &                 GPT-J &              OPT-6.7B &               OPT-13B &              GPT-NeoX &               OPT-30B \\
\midrule
PIQA              &  \textbf{0.22} (0.00) &  \textbf{0.29} (0.00) &           0.22 (0.09) &  \textbf{0.31} (0.00) &  \textbf{0.34} (0.00) &  \textbf{0.22} (0.00) \\
BoolQ   &  \textbf{0.50} (0.00) &  \textbf{0.46} (0.00) &           0.19 (0.06) &           0.08 (0.25) &  \textbf{0.20} (0.00) &  \textbf{0.39} (0.00) \\
RTE     &  \textbf{0.19} (0.00) &  \textbf{0.38} (0.00) &  \textbf{0.30} (0.00) &  \textbf{0.34} (0.00) &  \textbf{0.25} (0.00) &           0.13 (0.09) \\
WIC     &  \textbf{0.12} (0.03) &           0.12 (0.14) &  \textbf{0.37} (0.00) &  \textbf{0.17} (0.03) &           0.08 (0.31) &  \textbf{0.28} (0.00) \\
WSC     &  \textbf{0.26} (0.00) &  \textbf{0.18} (0.01) &           0.07 (0.61) &           0.08 (0.34) &  \textbf{0.16} (0.02) &           0.12 (0.14) \\
\midrule
CB      &  \textbf{0.17} (0.00) &  \textbf{0.28} (0.00) &  \textbf{0.37} (0.00) &  \textbf{0.17} (0.00) &           0.04 (0.50) &  \textbf{0.32} (0.00) \\
Arc (Challenge) &  \textbf{0.28} (0.00) &  \textbf{0.38} (0.00) &           0.17 (0.05) &  \textbf{0.29} (0.00) &  \textbf{0.31} (0.00) &           0.17 (0.05) \\
Arc (Easy)      &  \textbf{0.23} (0.00) &  \textbf{0.40} (0.00) &  \textbf{0.24} (0.01) &  \textbf{0.27} (0.00) &           0.15 (0.06) &           0.11 (0.19) \\
Hellaswag         &  \textbf{0.34} (0.00) &  \textbf{0.42} (0.00) &  \textbf{0.35} (0.00) &  \textbf{0.37} (0.00) &  \textbf{0.48} (0.00) &  \textbf{0.41} (0.00) \\
OpenBookQA        &  \textbf{0.23} (0.00) &  \textbf{0.50} (0.00) &  \textbf{0.27} (0.00) &  \textbf{0.40} (0.00) &  \textbf{0.42} (0.00) &  \textbf{0.23} (0.01) \\
\bottomrule
\end{tabular}

\end{sc}
% \end{small}
\end{center}
\vskip -0.1in
\end{table*}



==> fables/tab_highprompts.tex <==
\begin{table}[hb]
\caption{High-influence examples sampled from the top 20 (most positive) and bottom 20 (most negative) percentile bin for GPT-NeoX.}
\label{tab_highprompts}
\vskip 0.1in
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Task} & \textbf{\begin{tabular}[c]{@{}l@{}}Influence\\ Percentile\end{tabular}} & \textbf{ID} & \textbf{Prompt} \\ \midrule
PIQA  & 0 & 12444 & \begin{tabular}[c]{@{}l@{}}Goal: flashlight\\ Answer: shines a light\end{tabular} \\
 & 90 & 4286 & \begin{tabular}[c]{@{}l@{}}Goal: To bind fabric before putting it through a sewing machine.\\ Answer: You should use small pins.\end{tabular} \\
 \midrule
BoolQ & 0 & 2445 & \begin{tabular}[c]{@{}l@{}}1:64 scale -- Currently, 1:64 scale is most commonly used for automobile and other vehicle models, but it is also a popular scale for model railroads and toy trains... \textbackslash\\ In addition, 28mm military and fantasy figures are a popular size for tabletop gaming...\\ question: the ratio of the model cars dimensions to the actual cars dimensions is 1 56?\\ answer: no\end{tabular} \\
 & 90 & 6246 & \begin{tabular}[c]{@{}l@{}}My Mad Fat Diary -- After three series and sixteen episodes, My Mad Fat Diary broadcast its final episode on 6 July 2015.\\ question: will there be a season 4 of my mad fat diary?\\ answer: no\end{tabular} \\
\midrule
WIC & 0 & 2999 & \begin{tabular}[c]{@{}l@{}}Pull a bank robbery.\\ He regularly pulls 12-hour days, sometimes 14.\\ question: Is the word `pull' used in the same sense in the two sentences above?\\ answer: true\end{tabular} \\
 & 90 & 4298 & \begin{tabular}[c]{@{}l@{}}He longed for the touch of her hand.\\ This room needs a woman's touch.\\ question: Is the word `touch' used in the same sense in the two sentences above?\\ answer: false\end{tabular} \\
\midrule
WSC & 0 & 272 & \begin{tabular}[c]{@{}l@{}}Passage: We had hoped to place copies of our newsletter on all the chairs in the auditorium, but there were simply too many of them .\\ Question: In the passage above, does the pronoun `them' refer to chairs?\\ Answer: true\end{tabular} \\
 & 90 & 228 & \begin{tabular}[c]{@{}l@{}}Passage: Sam took French classes from Adam , because he was known to speak it fluently.\\ Question: In the passage above, does the pronoun 'he' refer to Adam?\\ Answer: true\end{tabular} \\
\midrule
Arc (Challenge) & 0 & 213 & \begin{tabular}[c]{@{}l@{}}Question: Which unit is used to record distances between stars?\\ Answer: light years\end{tabular} \\
 & 90 & 325 & \begin{tabular}[c]{@{}l@{}}Question: Which of these is a function of all cells?\\ Answer: to extract energy from food to sustain life\end{tabular} \\
\midrule
Arc (Easy) & 0 & 1052 & \begin{tabular}[c]{@{}l@{}}Question: A farmer sprayed his orange trees with a pesticide to eliminate the insects damaging the trees. \textbackslash\\ Some of the insects survived and produced offspring that were also resistant to the insecticide. \textbackslash\\ Which process is illustrated by the pesticide resistance of the offspring?\\ Answer: natural selection\end{tabular} \\
 & 90 & 1340 & \begin{tabular}[c]{@{}l@{}}Question: Modern technology has had some positive and negative effects on society. Which would be a negative effect of advances in technology?\\ Answer: human jobs replaced by more efficient machines\end{tabular} \\
\midrule
OpenBookQA & 0 & 3206 & \begin{tabular}[c]{@{}l@{}}Context: which one of these is false about the greenhouse effect?\\ Answer: it causes green air in the sky\end{tabular} \\
 & 90 & 3756 & \begin{tabular}[c]{@{}l@{}}Context: One of the reasons some species go extinct is because predators\\ Answer: murder too many of them\end{tabular} \\ \bottomrule
\end{tabular}
}
\end{center}
\end{table}

==> fables/tab_taskmodelaccuracy.tex <==
\begin{table*}[b]
\caption{Classification accuracy for each task-model pair. Bolded number marks the model that performs the best on a particular task.}
\label{tab_taskmodelaccuracy}
\vskip 0.1in
\begin{center}
\begin{tabular}{lrrrrrr}
\toprule
task &  GPT2-XL &  GPT-J &  OPT-6.7B &  OPT-13B &  GPT-NeoX &  OPT-30B \\
\midrule
piqa              &     75.2 &   \textbf{79.5} &      77.2 &     78.8 &      77.9 &     77.4 \\
superglue boolq   &     54.5 &   63.4 &      64.8 &     \textbf{70.5} &      68.9 &     70.3 \\
superglue rte     &     52.3 &   54.9 &      55.5 &     51.8 &      61.8 &     \textbf{64.9} \\
superglue wic     &     49.9 &   54.2 &      52.3 &     \textbf{54.5} &      52.1 &     54.4 \\
superglue wsc     &     40.0 &   49.8 &      57.4 &     \textbf{58.8} &      47.7 &     55.1 \\
\midrule
superglue cb      &     33.0 &   \textbf{47.8} &      29.6 &     35.7 &      34.4 &     39.7 \\
ai2 arc (challenge) &     30.0 &   36.6 &      35.4 &     36.6 &      39.5 &     \textbf{39.6} \\
ai2 arc (easy)      &     61.1 &   71.8 &      71.9 &     73.4 &      \textbf{77.5} &     75.3 \\
hellaswag         &     37.2 &   48.7 &      46.6 &     51.4 &      \textbf{54.7} &     54.5 \\
openbookqa        &     24.7 &   32.1 &      32.8 &     \textbf{34.4} &      \textbf{34.4} &     32.6 \\
\bottomrule
\end{tabular}
\end{center}
\vskip -0.1in
\end{table*}

==> fables/tab_topcommon.tex <==
\begin{table}[htb]
\caption{Number of examples shared between the respective top and bottom 20 percentile bins of influences for models in the same family. GPT-Neo family shares more common high-influence points compared to OPT family.}
\label{tab_topcommon}
\vskip 0.1in
\begin{center}
% \begin{small}
\begin{sc}
% \begin{tabular}{llrr}
% \toprule
%  family &            task & bottom & top \\
% \midrule
% GPT-Neo &            PIQA &     24 &  27 \\
% &           BoolQ &     18 &  16 \\
% &             RTE &     15 &  13 \\
% &             WIC &     36 &  29 \\
% &             WSC &     30 &  21 \\
% &              CB &     11 &  12 \\
% & Arc (Challenge) &     20 &  21 \\
% &      Arc (Easy) &     19 &  22 \\
% &       Hellaswag &     36 &  30 \\
% &      OpenBookQA &     34 &  34 \\
% \midrule
%     OPT &            PIQA &      6 &  11 \\
% &           BoolQ &      4 &  13 \\
% &             RTE &      3 &   5 \\
% &             WIC &     12 &  10 \\
% &             WSC &      5 &   6 \\
% &              CB &      3 &   4 \\
% & Arc (Challenge) &      6 &   4 \\
% &      Arc (Easy) &      9 &  13 \\
% &       Hellaswag &     18 &  20 \\
%  &      OpenBookQA &     20 &  17 \\
% \bottomrule
% \end{tabular}

\begin{tabular}{@{}lllllr@{}}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{}} & \multicolumn{1}{c}{\multirow{2}{*}{Total Count}} & \multicolumn{2}{c}{Bottom} & \multicolumn{2}{c}{Top} \\ \cmidrule(l){3-6} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{OPT} & \multicolumn{1}{c}{GPT-Neo} & \multicolumn{1}{c}{OPT} & \multicolumn{1}{c}{GPT-Neo} \\ \cmidrule(r){1-6}
PIQA & 80 & 6 & 24 & 11 & 27 \\
BoolQ & 80 & 4 & 18 & 13 & 16 \\
RTE & 80 & 3 & 15 & 5 & 13 \\
WIC & 80 & 12 & 36 & 10 & 29 \\
WSC & 80 & 5 & 30 & 6 & 21 \\
\midrule
CB & 50 & 3 & 11 & 4 & 12 \\
Arc (Challenge) & 80 & 6 & 20 & 4 & 21 \\
Arc (Easy) & 80 & 9 & 19 & 13 & 22 \\
Hellaswag & 80 & 18 & 36 & 20 & 30 \\
OpenBookQA & 80 & 20 & 34 & 17 & 34 \\ \bottomrule
\end{tabular}

\end{sc}
% \end{small}
\end{center}
\vskip -0.1in
\end{table}
